On the convergence of single-call stochastic extra-gradient methods

Variational inequalities have recently attracted considerable interest in machine learning as a flexible paradigm for models that go beyond ordinary loss function minimization (such as generative adversarial networks and related deep learning systems). In this setting, the optimal $\mathcal{O}(1/t)$ convergence rate for solving smooth monotone variational inequalities is achieved by the Extra-Gradient (EG) algorithm and its variants. Aiming to alleviate the cost of an extra gradient step per iteration (which can become quite substantial in deep learning applications), several algorithms have been proposed as surrogates to Extra-Gradient with a \emph{single} oracle call per iteration. In this paper, we develop a synthetic view of such algorithms, and we complement the existing literature by showing that they retain a $\mathcal{O}(1/t)$ ergodic convergence rate in smooth, deterministic problems. Subsequently, beyond the monotone deterministic case, we also show that the last iterate of single-call, \emph{stochastic} extra-gradient methods still enjoys a $\mathcal{O}(1/t)$ local convergence rate to solutions of \emph{non-monotone} variational inequalities that satisfy a second-order sufficient condition.

==> Algorithms/MG.tex <==
%----------------------------------------------------------------------
%%% META-GRADIENT
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\small
\tt
\begin{algorithmic}[1]
%\Require
%	feasible region $\points$, step-size sequence $\current[\step]>0$
\State
	initialize $\state_{\laststart} = \state_{\start} \in \points$,
	$\vecfield_{\paststart} = 0$
%	get oracle feedback $\vecfield_{\paststart}$
	\Comment{initialization}%
%\State
%	get oracle feedback $\vecfield_{\paststart}$ on $\state_{\paststart}$
%	\Comment{initialization}%
\For{$\run=\running$}
%	\State
%		oracle query at $\state$ returns $\gvec$
%		\Comment{gradient feedback}%
	\State
		generate $\inter$
		\Comment{leading state}%
	\State
		get $\inter[\vecfield]$ by oracle query at $\inter$
		\Comment{oracle feedback}%
	\State
		update $\current \leftarrow \update$
		\Comment{update base state}%
\EndFor
%\State
%	\Return $\state$
\end{algorithmic}


==> App-Exp.tex <==
Here we describe our experimental setup for the results presented in \cref{fig:ills}.
Let us consider a saddle-point problem on $\points=\R^{2\vdimalt}$ of the form
\begin{equation}
    \sadobj(\minvar,\maxvar) = \frac{\indic_1}{2}\minvar^\top\matmin_1\minvar
              + \frac{\indic_2}{4}(\minvar^\top\matmin_2\minvar)^2
              - \frac{\indic_1}{2}\maxvar^\top\matmax_1\maxvar
              - \frac{\indic_2}{4}(\maxvar^\top\matmax_2\maxvar)^2
              + \minvar^\top\matlin\maxvar,
\end{equation}
where $\minvar,\maxvar\in\R^\vdimalt$, $\indic_i\in\{-1, 0, 1\}$ for $i\in\{1, 2\}$, $\matlin\in\R^{\vdimalt\times\vdimalt}$ and
$\matmin_1, \matmin_2, \matmax_1, \matmax_2 \in \mathbb{S}^\vdimalt_{++}$ are positive definite matrices.
In our experiments, the ``coupling'' matrix $\matlin$ is generated randomly with i.i.d. entries drawn from the uniform distribution on $[0, 1/\vdimalt]$.
To obtain a positive definite matrix $\posmat$, we first generate a $\vdimalt\times\vdimalt$ random matrix $\randmat$ in the same way as $\matlin$, and then set $\posmat\defeq\randmat\randmat^\top+\minvalp\idm$ for some $\minvalp>0$.
This scheme is thus used to generate $\matmin_1, \matmin_2, \matmax_1, \matmax_2$ and we fix a same $\minvalp$ for the four matrices.
\ac{EG} and \ac{SEG} are both initialized at with the unit vector $(1/\sqrt{d}\thinspace\ldots~1/\sqrt{d})$ and $\state_\paststart=\state_\start$.
We take $\noise_\run$ as a white Gaussian noise of standard deviation $\noisedev$.
The three figures then correspond to the three following settings:
%
\begin{enumerate}[leftmargin=2em]
    \item [1.]\textbf{Deterministic strongly monotone.}~ $\indic_1=1$, $\indic_2=0$, $\vdimalt=1000$, $\minvalp=0.001$, $\noisedev=0$.
    \item [2.]\textbf{Deterministic monotone.}~ $\indic_1=0$, $\indic_2=1$, $\vdimalt=1000$, $\minvalp=0.001$, $\noisedev=0$.
    \item [3.]\textbf{Stochastic non-monotone.}~ $\indic_1=1$, $\indic_2=-1$, $\vdimalt=100$, $\minvalp=0.1$, $\noisedev=0.1$, $\gamma=10$.
\end{enumerate}
%
It is easy to verified that for the first two problems the point $0$ is the unique solution of \eqref{eq:SVI} and for the third problem $0$ is a regular solution of \eqref{eq:SVI}.

% \begin{table}[t]
%   \begin{center}
%   \caption{Parameters in different settings.}
%   \label{tab: cbs-res}
%     \begin{tabular}{l*{5}{>{$}c<{$}}}
%       \toprule
%       & \indic_1 & \indic_2 & \vdimalt & \minvalp & \noisedev \\
%       \midrule\\[-1em]
%       1. Deterministic strongly monotone
%       & 1 & 0 & 1000 & 0.001 & 0 \\
%       2. Deterministic monotone
%       & 0 & 1 & 1000 & 0.001 & 0 \\
%       3. Stochastic non-monotone
%       & 1 & -1 & 1000 & 1 & 0.05 \\
%       \bottomrule
%     \end{tabular}
%   \end{center}
% \end{table}

==> App-Merit.tex <==
\YGH{To be organized.}
For intuition, we discuss below the relation of the error function $\err(\test)$ to other performance measures that arise in practice (similar considerations apply to $\reserr$):
\begin{enumerate}[leftmargin=2em)]
%[\itshape a\upshape)]
\item
If $\vecfield = \nabla\obj$ for a convex differentiable function $\obj$ with $\inf_{\point\in\points}\obj(\point) > -\infty$, we have, for all $\point\in\points$, $\braket{\nabla\obj(\point)}{\test - \point} \leq \obj(\test) - \obj(\point)$, so $\err(\test) \leq \sup_{\point} \bracks{\obj(\test) - \obj(\point)} \leq \obj(\test) - \inf\obj$.
\item
In \acl{SP} problems, the quality of a candidate solution $\test = (\test[\minvar],\test[\maxvar])$ is often assessed via the \acdef{NI} function \citep{NK55}, defined here as
\begin{equation}
\label{eq:NI}
\tag{NI}
\nikiso(\test)
	= \sup_{\maxvar\in\maxvars} \sadobj(\test[\minvar],\maxvar)
	- \inf_{\minvar\in\minvars} \sadobj(\minvar,\test[\maxvar])
\end{equation}
provided of course that the \acl{RHS} is well-posed.
Similarly to the minimization framework above, if $\sadobj$ is convex-concave, we have $\err(\test) \leq \nikiso(\test)$.
\end{enumerate}
%Below we will consider that $\err$ is defined as $\nikiso$ for saddle-point problems.

==> App-Others.tex <==
%----------------------------------------------------------------------
%%% APP: VARIANTS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


\section{Previous presentation of the variants of Extra Gradient}
\label{sec:synthpres}




\ac{EG} \cite{Kor76}

\begin{equation}
%\label{eq:EG}
\begin{cases}
    \inter = \proj_{\points}(\current - \current[\step]\vecfield(\current)),\\
    \update = \proj_{\points}(\current - \current[\step]\vecfield(\inter)).
\end{cases}
\end{equation}

\ac{PEG} \cite{Pop80,GBVV+19}

\begin{equation}
%\label{eq:PEG}
\begin{cases}
    \inter = \proj_{\points}(\current - \current[\step]\vecfield(\past)),\\
    \update = \proj_{\points}(\current - \current[\step]\vecfield(\inter)).
\end{cases}
\end{equation}

\YGH{We initialize with $\state_{\paststart}$ and $\state_{\start}$ because this simplify the proof.}

\ac{OG} \cite{DISZ18}
\begin{equation}
%\label{eq:OGDA_orig}
    \update = \proj_{\points}(
        \current - 2\current[\step]\vecfield(\current) + \current[\step]\vecfield(\last)).
\end{equation}

\ac{OG} can also be written in the form:

\begin{equation}
%\label{eq:OGDA}
\begin{cases}
    \inter = \proj_{\points}(\current - \current[\step]\vecfield(\past)),\\
    \update = \inter - \current[\step]\vecfield(\inter) + \current[\step]\vecfield(\past).
\end{cases}
\end{equation}

Notice that here $\inter$ plays the role of $\current$ in \eqref{eq:OGDA_orig}.
\YGH{Past version of FBF}

\ac{RG} \cite{Mal15}

\begin{equation}
%\label{eq:RG_orig}
    \update = \proj_{\points}(
        \current - \current[\step]\vecfield(2\current-\last)).
\end{equation}

\YGH{Initialization with $\state_{\start}$ and $\state_{\laststart}$.}

It is equivalent to the following update:

\begin{equation}
\begin{cases}
    \inter = 2\current-\last,\\
    \update = \proj_{\points}(\current - \current[\step]\vecfield(\inter)).
\end{cases}
\end{equation}

We see that \ac{PEG}, \ac{OG} and \ac{RG} are equivalent without projection. 


==> Experiments.tex <==
%----------------------------------------------------------------------
%%% EXPERIMENTS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex



